The Unheralded Value of the Multiway Rendezvous: Illustration with the Production Cell Benchmark

The multiway rendezvous introduced in Theoretical CSP is a powerful paradigm to achieve synchronization and communication among a group of (possibly more than two) processes. We illustrate the advantages of this paradigm on the production cell benchmark, a model of a real metal processing plant, for which we propose a compositional software controller, which is written in LNT and LOTOS, and makes intensive use of the multiway rendezvous.

==> eptcsdata.tex <==
\providecommand{\firstpage}{230}
\providecommand{\publicationstatus}{H. Hermanns, P. H\"ofner (Eds.): Models for \\
Formal Analysis of Real Systems (MARS 2017)\\
EPTCS 244, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.244.10}{10.4204/EPTCS.244.10}}

